Towards Greener Applications: Enabling Sustainable Cloud Native Applications Design

Data centers energy demand is increasing. While a great deal of effort has been made to reduce the amount of CO$_2$ generated by large cloud providers, too little has been done from the application perspective. We claim that application developers can impact the environmental footprint by enhancing the application design with additional features. Following the proposed Sustainable Application Design Process (SADP), the application design is enriched with information that can be leveraged by cloud providers to manage application execution in an energy-aware manner. This exploratory work aims to emphasize the awareness on the sustainability of applications by proposing a methodology for its evaluation. To this end, we first suggest possible actions to enrich the application design towards sustainability, and finally describe how this additional information can be leveraged in the application workflow. We discuss the feasibility of our methodology by referring to existing tools and technologies capable of supporting the design features proposed in a production environment.

==> motivation_and_approach.tex <==






==> sections/maturitymodel.tex <==

\section{Sustainable Application Design Process}
\label{sec:maturity}

The proposed Sustainable Application Design Process (SADP) aims at supporting designers in the achievement of sustainable microservice based applications. SADP focuses on an application perspective by providing goals and directions for designing sustainable applications.
The following steps have been identified:% (Fig.~\ref{fig:samm}):

\begin{itemize}
    \item \textbf{Step 0: No Progress.} No action is taken by the application designer to improve the sustainability of an application.
    \item \textbf{Step 1: Sustainability Awareness.} The design of the components of the application is enriched with additional information regarding the resource requirements, QoS constraints, and power consumption for execution.
    \item \textbf{Step 2: Microservice Classification.} In this step, components should be annotated with their relevance for the overall application. Components are distinguished in mandatory for the success of the application and optional even though improving the QoE or the QoS of the final customer. 
    \item \textbf{Step 3: Microservices Enrichment.} For each activity, different modalities of execution might be defined according to their impact on energy consumption. For instance, normal, high quality, and low power mode can be defined. A sustainable workflow design recommends alternative modalities that can be selected according to the context of execution.
    %\item \textbf{Step 4: Sustainability Native Microservices.} Microservices are re-designed from scratch in order to ensure a higher efficiency in the usage of resources and a native ability to adapt to different environmental condition in order to reduce the CO$_2$ emissions.
\end{itemize}


% \begin{figure*}[!t]
% \centering
% \includegraphics[width=.8\textwidth]{figures/SAMM.pdf} 
% \caption{The SADP steps}\label{fig:samm}
% \end{figure*}

At \textbf{Step 0}, the application designer is not putting effort in designing sustainable applications. Level 0 is the current state of the art, where most focus is given to QoS while sustainability is mainly disregarded. 

\textbf{Step 1} is a first step towards sustainable applications. It consists in adding basic sustainability-aware information to the application design. The goal is to enrich the application model with additional information that can drive the deployment decisions of the cloud provider when the single components are deployed. This information is not only related to the energy aspect, but also to functional and QoS requirements. To lead towards an effective deployment, each application component (microservice) has to be complemented with metadata regarding the amount of required resources (e.g., the size of the VM required for deploying that component), QoS requirements (e.g., response time or throughput constraints), and power profiling (e.g., the estimated power consumption for executing the microservice). This last point is not trivial, since providing such information is not straightforward. However, from a simple profiling activity it is possible to estimate the computational power required by a specific VM or container configuration. Models available in the state of the art, transforming computational power in energy consumption, can then be exploited \cite{brondolin_deep-mon_2018}. A score can be assigned to the application measuring the extent to which the application design implements SADP's Step 1 best practices. The score is assigned according to the coverage of the annotation (i.e, how many of the suggested metadata are provided during the annotation process). 

An application designed according to \textbf{Step 2} provides information on which components of the application are mandatory and which are optional. Considering the flight reservation application example in Fig.~\ref{fig:app}, the rental car service can provide additional value for the customer and additional revenue for the application owner, but it is not a key component of the main application. If information about the relevance of each component is provided at design time, this information can be exploited to decide when to execute or when to skip a component according to the execution context. This information is relevant not only for the sustainability of the application (e.g., skip an optional component when renewable power source is not available), but also for QoS (e.g., avoid optional components when the application is experiencing response time or latency issues). Two possible approaches can be used to implement Step 2: i) all components require annotations stating if they are necessary or not for the overall workflow, ii) only optional components are annotated, while mandatory components are not explicitly identified. In the first case, a score can be assigned according to the amount of components explicitly annotated in the workflow. However, this approach is more time consuming. In the second approach, instead, a refined score cannot be associated, since it is not possible to differentiate between not annotated and implicitly annotated components. Thus, for the second approach, the score can only be 0 if no annotation is provided, and 1 if at least one component has been annotated as optional.

\textbf{Step 3} of the proposed SADP, consists in the enrichment of the microservices composing the application through the definition of different modalities of execution for each component. Alternative execution modalities can be defined for a single microservice and the one to enact might depend on the current context. Here, we propose three different execution modalities:
\begin{itemize}
    \item Normal: this is the basic execution modality of the microservice;
    \item High-Performance: in this modality, the performance of the microservice is stressed so that the QoS and/or QoE of the customer is maximized at the cost of a higher computational resource demand and power comsumption;
    \item Low-power: it is a simplified version of the microservice aiming at reducing the amount of energy consumed. To guarantee the performance level, some sub-activities are skipped or executed differently. As an example, in the flight reservation application, the ``Search flight'' component might take into account the previous activities of the customer in ranking the results to provide a better QoE. However, this has an additional computational cost that can be reduced by ignoring specific user information. 
\end{itemize}
\noindent For each microservice, both optional and mandatory, it is possible to define a low-power and a high-performance version. A score can be assigned according to the number of alternative versions provided compared to the overall amount of required versions. Different modalities correspond to different power consumption, QoS, and QoE for the customers, thus a trade-off is to be considered when selecting the proper modality.
%The last step of the proposed approach, \textbf{Step 4}, requires a total re-design of the microservices composing the application. This step guarantees the best results by natively considering energy efficiency and sustainability in the design process. However, it might be too expensive and time consuming and requires specific expertise that might not be available to the application's designer. In this step, the score is the percentage of microservices that have been re-designed. 
The overall SADP approach and the suggested best practices are summarized in Tab.~\ref{tab:samm}. It is worth noticing that the four steps are incremental refinements. At each step, additional information is provided by the application designer and, at the same time, the complexity in the management of the application increases since the degree of freedom of how to execute the application and its components is higher. Moreover, the process is incremental, since at each loop, the designer can focus on a single component or on a subset of components, enriching the model step by step.


\begin{table}[!t]
\scriptsize
\rowcolors{1}{}{lightgray}
\caption{SAMM description}
\label{tab:samm}
\begin{tabularx}{\textwidth}{ l | l | X | X }
  \toprule
  \textbf{Step} & \textbf{Name} & \textbf{Action} & \textbf{Score} \\
  \midrule 
  Step 0  & No action  & --  & --  \\
  \midrule 
  Step 1  & Sustainability Awareness  & Add metadata on requirements, QoS, and energy usage  & Coverage (0--100 \%)  \\
  \midrule 
  Step 2  & Microservice Classification  & Annotate components according to their relevance for the business goal & Coverage (0--100 \%) if explicit -- 0/1 if implicit \\
 \midrule 
  Step 3  & Microservice Enrichment  & Provide alternative modalities of execution for the components of the application  & Coverage (0--100 \%)  \\
  %\midrule 
  %Level 4  & Sustainability Native Microservices  & Re-design microservices to be sustainable by design  & Coverage (0--100 \%)  \\
  \bottomrule
\end{tabularx}
\end{table}
